Online Dynamic Acknowledgement with Learned Predictions

We revisit the online dynamic acknowledgment problem. In the problem, a sequence of requests arrive over time to be acknowledged, and all outstanding requests can be satisfied simultaneously by one acknowledgement. The goal of the problem is to minimize the total request delay plus acknowledgement cost. This elegant model studies the trade-off between acknowledgement cost and waiting experienced by requests. The problem has been well studied and the tight competitive ratios have been determined. For this well-studied problem, we focus on how to effectively use machine-learned predictions to have better performance. We develop algorithms that perform arbitrarily close to the optimum with accurate predictions while concurrently having the guarantees arbitrarily close to what the best online algorithms can offer without access to predictions, thereby achieving simultaneous optimum consistency and robustness. This new result is enabled by our novel prediction error measure. No error measure was defined for the problem prior to our work, and natural measures failed due to the challenge that requests with different arrival times have different effects on the objective. We hope our ideas can be used for other online problems with temporal aspects that have been resisting proper error measures.

==> 60_lowerbound.tex <==
\subsection{Lower Bound}
\label{sec:lowerbound}

In this section, we mainly show a lower bound of the problem.
Recall the lower bound theorem \cref{thm:eta3:lowerbound}.

% \begin{theorem}
% Given an arbitrary instance $I$ of \DTAP/ and its prediction instance $\hatI$,
% the solution of any deterministic algorithm is at least $\min\{(1+\lambda-\epsilon)\cdot \opt(I),(\opt(I)+\frac{\eta}{\lambda}) \}$, where $\lambda>0$ is a constant and $\eta$ is the prediction error defined in \cref{def:eta3}.
% \label{thm:eta3:lowerbound}
% \end{theorem}

% \begin{proof}
% To show \cref{thm:eta3:lowerbound}, we consider the following hard instance.
% The predicted instance only has one time point and we assume that the number of packets is $p_1$, where $\frac{p_1}{d}=\epsilon$.
% The actual instance has $p_1$ packets at time $1$, and all the remaining time points have no packets.
% The actual instance may have $p_t$ packets at time $t$ depending on the algorithm's decision.
% Assume that an arbitrary algorithm $\alg$ sends an ack at the time $t'$.
% Let $D(p_1)$ be the delay of the packets in time $1$ in $\alg$'s solution.
% If $D(p_1)\geq \lambda - \epsilon$, then we set $p_t=0$ in the actual instance, i.e., the actual instance only has $p_1$ packets in time $1$.
% Clearly, $\alg(I)\geq \lambda+1-\epsilon$ while $\opt(I)=1$.
% Thus, $\alg(I)\leq (\lambda+1-\epsilon)\cdot \opt(I)$ in the current case.
% If $D(p_1)<\lambda - \epsilon$, set $t=t'+1$, i.e., the actual instance has $p_{t'+1}$ packets in the time $t'+1$.
% Clearly, $\alg(I)\geq 2+ D(p_1)$.
% By the definition of $\eta$, we have $\eta=\sD(p_1)+\epsilon$ since $\opt(\dO(I,\hatI))=\opt(I)=1+\sD(p_1)+\epsilon$ and $\opt(\dU(I,\hatI))=\opt(\hatI)=1$.
% Thus, $\alg(I)\geq\opt(I)+1$ since $\sD(p_1)=\epsilon$.
% Since $\sD(p_1)<\lambda-\epsilon$, we have $\frac{\eta}{\lambda}<1$.
% Thus, we have $\alg(I)\geq \opt(I)+\frac{\eta}{\lambda}$.
% \end{proof}




==> 70_learnability.tex <==
\subsection{Learnability}
    \label{sec:app_learnable}


% In this section, we show the learnability of our prediction by proving that given only a polynomial number of samples, we can learn a prediction whose expected error is nearly minimum. 
% In the following, we always assume that the number of time steps is at most $T$, the number of packages per time step is at most $K$ and each TCP instance is sampled from an unknown distribution $\cD$.
% Use $\cI$ to denote the set of all potential predictions $\hatI$, i.e., $\cI:=\set{(p_1,p_2,...,p_T)\mid\forall t\in [T], p_t\in [0,K]}$.

% \begin{theorem}\label{thm:learnability}
% For any $\epsilon,\delta \in (0,1)$ and any distribution $\cD$, after observing $O((\frac{T}{\epsilon})^2(T\log(\frac{KT}{\epsilon d})+\ln(\frac{1}{\delta}))$ samples, there exists a learning algorithm that returns a predicted instance $\hatI \in \cI$ such that with probability at least $1-\delta$,
%     \[\E_{I \thicksim \cD}[\eta(\hatI,I)] \leq \E_{I \thicksim \cD}[\eta(I^*,I)] + \epsilon, \]
%     where for any two instances $I_1,I_2$, $\eta(I_1,I_2)$ represents the error when $I_1$ is the prediction of $I_2$, and $I^* = \argmin_{I'\in \cI}\E_{I \thicksim \cD}[\eta(I',I)]$.
% \end{theorem}


% The basic idea of this proof is that we first show that with only a small loss on the minimum expected error, $\cI$ can be reduced to a finite set.
% Then due to the bounded pseudo-dimension of that finite set, the sample complexity can be bounded.
% Before stating the reduction, we prove a simple lemma first. 

% \begin{lemma}\label{lem:l1_norm}
% For any two instances $I_1=\{p_t^{(1)}\}_{t\in[T]}$ and $I_2=\{p_t^{(2)}\}_{t\in[T]}$, $|\opt(I_1)-\opt(I_2)|\leq \rho T/d$, where $\rho$ is the $\ell_1$-norm distance between the two instances. 
% \end{lemma}
% \begin{proof}
% Let $X^{(1)}$ be the optimal solution of instance $I_1$. 
% Let $\num X^{(1)}$ be the number of acknowledgements in solution $X^{(1)}$, and for each time point $t\in [T]$.
% Let $D_t^{(1)}$ denote the waiting time of the packages arriving at time $t$ in solution $X^{(1)}$. We have
% \begin{equation*}
%     \begin{aligned}
%     \opt(I_2) &\leq \sF(X^{(1)},I_2)\\
%     &=\num X^{(1)} + \sum_{t\in [T]} P_t^{(2)}D_t^{(1)}/d\\
%     &\leq \num X^{(1)} + \sum_{t\in [T]} P_t^{(1)}D_t^{(1)}/d + \rho T/d\\
%     &=\opt(I_1) + \rho T/d.
%     \end{aligned}
% \end{equation*}

% Analogously, we can also prove that $\opt(I_1)\leq \opt(I_2)+\rho T/d$.

% \end{proof}

% \begin{lemma}\label{lem:reduce_finite_set}
% For any $\epsilon\in (0,1)$ and any distribution $\cD$, there exists a finite set $\cF$ with size $O((\frac{KT^2}{\epsilon d})^T)$ such that
% \[\min_{\hatI \in \cF}\E_{I \thicksim \cD}[\eta(\hatI,I)] \leq \min_{\hatI \in \cI}\E_{I \thicksim \cD}[\eta(\hatI,I)] + \epsilon. \]
% \end{lemma}

% \begin{proof}
% Given an $\epsilon\in (0,1)$, define $\epsilon_0:=\epsilon d/T^2$.
% The finite set $\cF$ is defined to be a set of instance $I \in \cI$, in which the number of packages at any time point is an integral multiple of $\epsilon_0$. Clearly, the size of $\cF$ is $O( (K/\epsilon_0)^T)$. Now we show that for any instance $I\thicksim \cD$ and $\hatI\in \cI/\cF$, we can round instance $\hatI$ to an instance $\hatI'\in \cF$ such that $|\eta(\hatI,I)-\eta(\hatI',I)|\leq \epsilon$, which implies $\min_{\hatI \in \cF}\E_{I \thicksim \cD}[\eta(\hatI,I)] \leq \min_{\hatI \in \cI}\E_{I \thicksim \cD}[\eta(\hatI,I)] + \epsilon$ directly.

% Partition the interval $[0,K]$ into $\lceil K/\epsilon_0 \rceil$ sub-intervals $[0,\epsilon_0],(\epsilon_0,2\epsilon_0],...,((\lceil K/\epsilon_0 \rceil-1)\epsilon_0, \lceil K/\epsilon_0 \rceil\epsilon_0]$. For an instance $\hatI \in \cI/\cF$, we round each $p_t$ to the upper bound of the sub-interval that $p_t$ belongs to. Denote the new instance after rounding by $\hatI'$. Clearly, the $\ell_1$-norm distance between instance $\hatI$ and $\hatI'$ is at most $T\epsilon_0$.

% For convenience, let $I_i^O:=\dO(I_i,\hatI_i)$ and $I_i^U:=\dU(I_i,\hatI_i)$.
% Recalling that $\eta(\hatI, I) := \max_{P\in \cP} \sum_{I_i\in P}(\opt(I_i^O)-\opt(I_i^U))$, we define $P_0$ to be the partition which yields the value of $\eta(\hatI', I)$, i.e., $P_0 =\argmax_{P\in \cP} \sum_{I_i\in P}(\opt((I_i')^O)-\opt((I_i')^U))$. 
% Note that the $\ell_1$-norm distance between instance $\hatI$ and $\hatI'$ is at most $T\epsilon_0$.
% By \cref{lem:l1_norm}, we have
% \begin{equation*}
%     \begin{aligned}
%     \eta(\hatI',I)&= \sum_{I_i \in P_0}(\opt((I_i')^O)-\opt((I_i')^U)) \\
%     &\leq \sum_{I_i \in P_0}(\opt((I_i)^O)-\opt(I_i^U)) + T^2\epsilon_0/d\\
%     & \leq \eta(\hatI, I) + \epsilon.
%     \end{aligned}
% \end{equation*}
% We can also prove $\eta(\hatI,I)\leq \eta(\hatI',I)+\epsilon$ analogously. Finally, we have $|\eta(\hatI,I)-\eta(\hatI',I)|\leq \epsilon$, which completes the proof.
% \end{proof}

% Since $\cF$ is a finite set with size $O((\frac{KT^2}{\epsilon d})^T)$, its pseudo-dimension is $O(T\log(\frac{KT}{\epsilon d}))$. According to the theorem proposed in~\cite{DBLP:journals/siamcomp/GuptaR17}, we have the following lemma.

% \begin{lemma}\label{lem:finite_set_small_dimension}
% For any $\epsilon,\delta \in (0,1)$ and any distribution $\cD$, after observing $O((\frac{T}{\epsilon})^2(T\log(\frac{KT}{\epsilon d})+\ln(\frac{1}{\delta}))$ training samples, 
% the predicted instance $\hatI \in \cF$ with the minimum empirical error $\eta$ among the training samples satisfies
%     \[\E_{I \thicksim \cD}[\eta(\hatI,I)] \leq \E_{I \thicksim \cD}[\eta(I^*,I)] + \epsilon \]
%     with probability at least $1-\delta$, where $I^* = \argmin_{I'\in \cF}\E_{I \thicksim \cD}[\eta(I',I)]$.
% \end{lemma}

% Combining \cref{lem:reduce_finite_set} and \cref{lem:finite_set_small_dimension}, \cref{thm:learnability} can be proved directly.
